Large Language Model-guided Document Selection

Large Language Model (LLM) pre-training exhausts an ever growing compute budget, yet recent research has demonstrated that careful document selection enables comparable model quality with only a fraction of the FLOPs. Inspired by efforts suggesting that domain-specific training document selection is in fact an interpretable process [Gunasekar et al., 2023], as well as research showing that instruction-finetuned LLMs are adept zero-shot data labelers [Gilardi et al.,2023], we explore a promising direction for scalable general-domain document selection; employing a prompted LLM as a document grader, we distill quality labels into a classifier model, which is applied at scale to a large, and already heavily-filtered, web-crawl-derived corpus autonomously. Following the guidance of this classifier, we drop 75% of the corpus and train LLMs on the remaining data. Results across multiple benchmarks show that: 1. Filtering allows us to quality-match a model trained on the full corpus across diverse benchmarks with at most 70% of the FLOPs, 2. More capable LLM labelers and classifier models lead to better results that are less sensitive to the labeler's prompt, 3. In-context learning helps to boost the performance of less-capable labeling models. In all cases we use open-source datasets, models, recipes, and evaluation frameworks, so that results can be reproduced by the community.

==> tables/different_thresholds.tex <==
\begin{table}
  \caption{Comparisons of 1B models trained on Common Crawl (via Common Crawl (via the RedPajama dataset~\cite{together2023redpajama}) with different selection ratio. 100\% denotes no filter and 55\% shows that the documents with top 55\% scores are selected for training.. (may replace with a figure) }
  \label{tab:different_ratio}
  \centering
  \begin{tabular}{c | c  c c}
    \toprule
     Ratio (\%) & CoreEN (0S) & CoreEN (All) & MMLU \\
     \midrule
    100 &  57.44 &  47.80 & 24.49  \\
    55 & 59.22 & 49.50 & 24.62  \\
    45 & 60.27 & 50.42 & 24.38 \\
    35 &  60.33 & 50.35& 24.98  \\
    25 &   60.54 & 51.20 & 25.03 \\
    15 &  59.99 & 49.79 & 24.27 \\
     
    \bottomrule
  \end{tabular}
\end{table}
